Multi-Stage Pre-training for Low-Resource Domain Adaptation

Transfer learning techniques are particularly useful in NLP tasks where a sizable amount of high-quality annotated data is difficult to obtain. Current approaches directly adapt a pre-trained language model (LM) on in-domain text before fine-tuning to downstream tasks. We show that extending the vocabulary of the LM with domain-specific terms leads to further gains. To a bigger effect, we utilize structure in the unlabeled data to create auxiliary synthetic tasks, which helps the LM transfer to downstream tasks. We apply these approaches incrementally on a pre-trained Roberta-large LM and show considerable performance gain on three tasks in the IT domain: Extractive Reading Comprehension, Document Ranking and Duplicate Question Detection.

==> experiments_old.tex <==


%\begin{table*}[t]
%\centering
%\small
%\begin{tabular}{|l|cccc|cccc|}
%\hline
%   \textbf{Model} & \multicolumn{4}{c|}{\textbf{Dev}} & \multicolumn{4}{c|}{\textbf{Test}} \\
%   \hline
%  &\textbf{MAP} & \textbf{MRR} & \textbf{P@1} &\textbf{P@5} & \textbf{MAP} & \textbf{MRR} & \textbf{P@1} & \textbf{P@5} \\
%  \hline
%  RoBERTa & 0.6343 & 0.7328 & 0.5884 & 0.5143 & 0.6625 & 0.7779 & 0.6537 & 0.5097 \\
%   \hline
%   + Domain LM & 0.6465 & 0.7529 & 0.6222 & 0.5229 & 0.6767 & 0.7991 & 0.6763 & 0.5154 \\
%   \hline
%   + 5K Vocab Ext. & 0.6530 & 0.7503 & 0.6083 & 0.5318 & 0.6864 & 0.8173 & 0.7043 & 0.5170 \\
%   \hline
%    +DQD Pre-training & \textbf{0.6723} & \textbf{0.7745} & \textbf{0.6465} & \textbf{0.5481} & \textbf{0.7035} & \textbf{0.8246} & \textbf{0.7139} & \textbf{0.5322} \\
%   \hline
%\end{tabular}
%\caption{Experimental results on AskUbuntu-DQD task. Each row with a + refers to incremental upgrade over the previous row. P@1 and P@5 refers to Precision@1 and Precision@5 respectively.}
% \label{tab:AskUbuntu}
%\end{table*}
\begin{table*}[t]
\centering
\small
\begin{tabular}{l|cccc|cccc}
\hline
   \textbf{Model} & \multicolumn{4}{c|}{\textbf{Dev}} & \multicolumn{4}{c}{\textbf{Test}} \\
 
  &\textbf{MAP} & \textbf{MRR} & \textbf{P@1} &\textbf{P@5} & \textbf{MAP} & \textbf{MRR} & \textbf{P@1} & \textbf{P@5} \\
  \hline
  RoBERTa & 0.634 & 0.733 & 0.588 & 0.514 & 0.663 & 0.778 & 0.654 & 0.510 \\
   \hline
   + Domain LM & 0.647 & 0.753 & 0.622 & 0.523 & 0.677 & 0.799 & 0.676 & 0.515 \\
   
   + 5K Vocab Ext. & 0.653 & 0.750 & 0.608 & 0.532 & 0.686 & 0.817 & 0.704 & 0.517 \\
  
    +DQD Pretraining & \textbf{0.672} & \textbf{0.775} & \textbf{0.647} & \textbf{0.548} & \textbf{0.704} & \textbf{0.825} & \textbf{0.714} & \textbf{0.532} \\
   \hline
\end{tabular}
\caption{Experimental results on AskUbuntu-DQD task. Each row with a + refers to incremental upgrade over the previous row. P@1 and P@5 refer to Precision@1 and Precision@5 respectively.}
 \label{tab:AskUbuntu}
\end{table*}

\subsection{Setup}

%RoBERTa-large language model is used as the baseline model in our experiments. 
%\avi{I don't like the oob term, pls change the first sentence to: Our experiments build on top of the \roberta-large LM.}
%Our baseline experiments rely on an out-of-the-box \roberta-large LM. 

%\avi{Move this to appendix:} We use the Facebook Fairseq toolkit~\cite{ott2019fairseq} for language modelling and the HuggingFace Transformers library~\cite{Wolf2019HuggingFacesTS} for downstream tasks. 
%We continue pre-training RoBERTa-large on task specific data, TechQA Technotes and AskUbuntu, separately by using Facebook Seq-to-Seq Toolkit \footnote{https://github.com/pytorch/fairseq}.
Our experiments build on top of the \roberta-large LM.
We adopt the standard methodology of using the pre-trained LM as the encoder and processing the contextualized representations it produces using task-specific layers. For the TechQA-RC task, we follow~\cite{devlin-etal-2019-bert} and predict the start and end position of the answer span with two separate classifiers, trained using cross entropy loss. For the TechQA-DR and AskUbuntu-DQD tasks, we follow~\cite{adhikari2019docbert} and classify the [CLS] token representation at the final layer with a binary classifier trained using the binary cross entropy loss; during inference, we rank the documents or questions according to their classification score. 
%For the AskUbuntu-DQD task, we follow the same approach as TechQA-DR task, by using a classifier over the [CLS] output and using the classification score for ranking. 
For all the tasks, during finetuning, we train the entire model end-to-end. 

For the TechQA-RC task, we report both the main metric, F1, and the ancillary F1 for answerable questions, HA\_F1, to capture the effects of our approach both on the end-to-end pipeline (F1) and on the answer extraction component (HA\_F1). For TechQA-DR, models are evaluated by Match@1 and Match@5. For AskUbuntu-DQD, we report MAP, MRR, Precision@1 and Precision@5 following~\cite{lei-etal-2016-semi}.
%Our downstream modeling follows the methodology of \cite{devlin-etal-2019-bert}: evidence text is first organized into a sequence of tokens that is passed to the LM to produce contextual vector representation, then the encoded output is further fed into task-specific layers to solve target problem. If not explicitly stated otherwise, the last step of model training is the fine-tuning using the labeled data that each target task provides. 

%We run 5 seeds for each model training and report the average score.  For TechQA-DR, models are evaluated by Match@1 and 5. For AskUbuntu-DQD, 4 metrics are adopted following \cite{lei-etal-2016-semi}: MAP, MRR, Precision@1 and 5. The experimental results of TechQA are mostly reported for dev set because the policy of TechQA leaderboard doesn't allow frequent submission.



%For TechQA-QA, we construct a synthetic corpus from TechQA Technotes containing 115K positive examples, each of which has 10 randomly selected documents to form negative features. For AskUbuntu-DQD, a 210K-example synthetic corpus is constructed from the web dump data, in which the positive:negative example ratio is about 1:1.


\subsection{Synthetic Pre-training Corpus and Labeled Data Augmentation}

Using the method described in section \ref{section:synt}, we use the 801K Technotes to construct a synthetic corpus for the TechQA tasks. The synthetic data contains 115K positive examples, each of which has 10 randomly selected documents as negatives. For the AskUbuntu-DQD, a 210K-example synthetic corpus is constructed from the web dump data, with a positive:negative example ratio of 1:1.

Since TechQA is a very-low resource dataset with only 600 training examples, we additionally apply data augmentation techniques to increase the size of the training set. We use simple data perturbation strategies, such as adding examples with only parts of the original query, randomly dropping words in query and passage, duplicating positive examples, removing stop words, dropping document title in the input sequence etc., to increase the size of the training set by 10 times. 
%Only under the data augmentation setting, this augmented training set is used while fine-tuning on the TechQA tasks.
This augmented training set is only used under the
data augmentation setting while fine-tuning on the TechQA tasks.

%These include duplicating positive examples, dropping question and document titles from input sequence, removing stop words, and \avi{I don't understand this part:}
%randomly deleting words with a small rate from query and passage, which together increase the training set by 10 times.  A second round pre-training is performed on the augmented training set for TechQA tasks before final fine-tuning.




\subsection{Results and Analysis}

For each of our approaches, we show performance of the model when fine-tuned on the downstream tasks in TechQA and AskUbuntu datasets. All the numbers reported are averages over 5 seeds, 
unless otherwise stated.
\newline
%\rong{we need to mention the TechQA numbers discussed below are from dev set}

\noindent \textbf{TechQA-RC} 
Table~\ref{tab:QA} describes the performance on the RC task in the TechQA dataset. %The numbers on the blind test set were obtained from a single submission to the TechQA leaderboard~\footnote{} and
The BERT baseline numbers are from~\cite{castelli2019techqa}.
Here, model performance is compared on the dev set and we report the blind test set numbers\footnote{Obtained by submitting to the \href{https://leaderboard.techqa.us-east.containers.appdomain.cloud}{\textit{TechQA leaderboard}}} for our single-best baseline and final models.

%Model performances are compared based on dev set results because TechQA leaderboard doesn't allow frequent submission.

Adapting the LM without extending the vocabulary yields just 0.2 points over the \roberta-large baseline. Augmenting the vocabulary by 10k word pieces improves the HA\_F1 score by $1.7$ points. Furthermore, our RC-style synthetic pre-training yields a considerable improvement of 2.8 points on HA\_F1 and 0.5 points on F1. %, suggesting that the synthetic data helps the model gain domain knowledge.
Finally,  data augmentation further boosts performance by  $~1$ point on both HA\_F1 and F1, suggesting that data augmentation via simple perturbations \ can be effective in a very-low resource setting. \newline

%Starting from the RoBERTa-large LM, we carry out the LM and QA model pre-training with different settings. As illustrated by "Tech RoB.+0K" in Table \ref{tab:QA}, task-specific LM pre-training without enhancing vocabulary only achieves a small gain over the baseline RoBERTa-large. On the other hand, the method of vocabulary extension, illustrated by the Tech\_RoB.+10K, brings us substantial improvement especially on HasAnswer\_F1. This indicates that for a domain using different terminology, i.e. IT support, directly representing new words into LM is more effective than modeling them through BPE based contextual embeddings. Tech\_RoB.+10K LM is further trained on the 115K synthetic corpus for initializing QA layer. The effectiveness of the downstream model pre-training is shown by "+QA Pre-training", which improves the HasAnswer\_F1 by 2.80, and F1 by 0.54 on dev set, from Tech\_RoB.+10K.

%We additional apply data augmentation techniques to increase the size of the 600-example training set. These include duplicating positive examples, dropping question and document title from input sequence, removing stop words, and randomly deleting words, which together increase the training set by 10 times. A second round QA pre-training, using the "+QA Pre-training" as initial model, is performed on the augmented data. With the help of LM pre-training, 2 rounds of QA pre-training and final fine-tuning, we established STOA for TechQA leaderboard which outperforms the RoBERTa-large baseline significantly: 5.60 of HasAnswer\_F1 and 1.72 of F1 on dev set, and 2.84 of HasAnswer\_F1 and 2.99 of F1 on test set.

\noindent \textbf{TechQA-DR} 
Table \ref{tab:DR} shows results from our experiments on the auxillary document ranking task over the TechQA dataset. We use BM25 \cite{articleBM25} as our IR baseline.
%\revanthnote{@Vittorio: Can you better explain this sentence and maybe add a reference for BM25} \anthony{I added in the ref for bm25}. 
We see that the 
%transformer
RoBERTa
models substantially outperform the IR system. Although vocabulary expansion only helps by 0.3 points in  Match@1, 
%our other approaches yield 
%\avi{did you measure stat. significance else remove this term} significant
%additional gains.
we see considerable improvements in performance from our other approaches.
%\avi{I don't understand this sentence:} 
%We observe the additional Match@1 gains of 2.9 points from the "+QA pretraining" in a transfer learning settings, and the 1.3 additional points from data augmentation. 
The ``RC Pre-training" entry shows a Match@1 improvement of 2.9 points over the language modelling. This demonstrates the effectiveness of pre-training on an ancillary task in a transfer-learning setting for the document ranking task.
%The effectiveness of pre-training on an ancillary task in a transfer learning setting---the RC {Pre-training} entry---is evident in the improvement of 2.9 point in Match@1 for the document ranking task. 
We further see an improvement of 1.3 points from data augmentation.%\footnote{The numbers on the test set were obtained by the TechQA leaderboard manager who agreed to run our scoring script on an output file produced by our submission.}


%\begin{table}
%\centering
%\small
%\begin{tabular}{|l|cc|cc|}
%\hline
% \textbf{Model}& \multicolumn{2}{c|}{\textbf{Dev}} & \multicolumn{2}{c|}{\textbf{Test}} \\
%\hline
%   & \textbf{HA\_F1} & \textbf{F1} &  \textbf{HA\_F1} & \textbf{F1} \\
%   \hline
%   BERT  & 34.69 & 55.31 & 25.36 & 53.38 \\

%  RoBERTa & 34.95 & 58.16 & 29.29  & 54.92  \\

%  + Domain LM & 35.21 & 58.27 & - & -  \\

  %\hline
  %\hline
%   +10K Vocab Ext. & 36.89 & 58.50 & - & -  \\

%    +QA Pre-training & 39.69 & 59.04 & - & -\\

%     +Data Aug. & \textbf{40.55} & \textbf{59.88} & \textbf{32.13}  & \textbf{57.91} \\
%   \hline
%\end{tabular}
%\caption{Experiments on TechQA-QA task. BERT baseline is reported from \cite{castelli2019techqa}. Each row with a + refers to incremental upgrade over the previous row. HA\_F1 refers to F1 for answerable questions}
%  \label{tab:QA}
%\end{table}

\begin{table}[]
\centering
\small
\begin{tabular}{l|cc|cc}
\hline
 \textbf{Model}& \multicolumn{2}{c|}{\textbf{Dev}} & \multicolumn{2}{c}{\textbf{Test}} \\
 
   & \textbf{HA\_F1} & \textbf{F1} &  \textbf{HA\_F1} & \textbf{F1} \\
   \hline
   BERT  & 34.7 & 55.3 & 25.4 & 53.0 \\

  RoBERTa & 35.0 & 58.2 & 29.3  & 54.4  \\
\hline
  + Domain LM & 35.2 & 58.3 & - & -  \\

  %\hline
  %\hline
   +10K Vocab Ext. & 36.9 & 58.5 & - & -  \\

    +RC Pretraining & 39.7 & 59.0 & - & -\\

     +Data Aug. & \textbf{40.6} & \textbf{59.9} & \textbf{32.1}  & \textbf{56.7} \\
   \hline
\end{tabular}
\caption{Results on TechQA-RC task. Each row with a + adds a step to the previous one. HA\_F1 refers to F1 for answerable questions.}
  \label{tab:QA}
\end{table}



\begin{table}[]
\centering
\small
\begin{tabular}{l|cc|cc}
\hline
 \textbf{Model}& \multicolumn{2}{c|}{\textbf{Dev}} & \multicolumn{2}{c}{\textbf{Test}\tablefootnote{Since this is not the official task in the TechQA dataset, numbers on the test set were obtained by the TechQA leaderboard manager who agreed to run our scoring script on an output file produced by our submission.}} \\

    & \textbf{M@1} & \textbf{M@5}& \textbf{M@1} & \textbf{M@5} \\
   \hline
  IR & 0.437 & 0.637 & - & - \\

  RoBERTa & 0.576 & 0.770 & 0.512  & 0.748 \\
\hline
  + Domain LM  & 0.593 & 0.808 & - & - \\

   +10K Vocab Ext.  & 0.596 & 0.790 & - & - \\

    +RC Pretraining & 0.625 & 0.826  & - & -\\

    +Data Aug. & \textbf{0.638} & \textbf{0.850}& \textbf{0.536} & \textbf{0.808} \\
    \hline
\end{tabular}
\caption{Experimental results on TechQA-DR task. Each row with a + adds a step to the previous row. M@1 is short for Match@1 and M@5 for Match@5.}
  \label{tab:DR}
\end{table}

~

\noindent \textbf{AskUbuntu-DQD} 
Table \ref{tab:AskUbuntu} shows results for the 
%\avi{I think you acronym-ed this then why use the full form?} 
%duplicate question detection 
DQD
task on the AskUbuntu dataset. We see that our methods give incremental improvements in performance. Our final model is considerably better than the \roberta-large baseline on all four metrics. We see the biggest gain in performance from the synthetic pre-training task demonstrating its relevance to the DQD task.  For this dataset, we didn't explore data augmentation strategies because  it had a considerable number of training instances (see Table~\ref{tab:Datasets}) compared to the TechQA dataset. 

%Task-specific LM pre-training, starting from RoBERTa-large, is carried out on AskUbuntu web dump data with 2 settings: one using standard vocabulary and one using 5K additional tokens. The superior performance of vocabulary extension in LM pre-training is demonstrated by the results in Table \ref{tab:AskUbuntu}. The DQD model pre-training, using the "AskUbuntu\_RoBERTa+5K" as initial model, is conducted on the 210K-example synthetic corpus. Table \ref{tab:AskUbuntu} shows that significant improvement, evaluated on both dev and test sets by 4 metrics, is achieved by the downstream model pre-training.




==> related_work.tex <==
%Transfer learning is a machine learning technique that applies the knowledge gained from solving one task to a related task. One commonly used approach in NLP is to pre-train an initial model from a source dataset which usually has abundant training data, then fine-tune it on the target dataset \cite{min-etal-2017-question, chung-etal-2018-supervised, wiese-etal-2017-neural-domain}. Generating synthetic examples to augment insufficient training data has been explored for low resource settings. For QA tasks, \cite{golub-etal-2017-two, yang-etal-2017-semi, lewis-etal-2019-unsupervised} developed supervised or semi-supervised models to generate natural questions. For the DQD task, \cite{conf-ijcai-QiuH15} modeled the relevance between question and accepted answer to improve question retrieval. \cite{lei-etal-2016-semi} pre-trained their question encoder within an encoder-decoder framework designed for body-to-title generation. \cite{ruckle-etal-2019-neural} also considered the body-title structure of unlabeled questions in weak supervision. Recent progress of pre-trained LMs inspired researches to adapt these large scale models into specific domains \cite{alsentzer-etal-2019-publicly, Lee_2019, alex2019unsupervised}. \cite{gururangan2020dont} investigated domain-adaptive and task-adaptive pre-training and showed the effectiveness of both.

